DEnsity: Open-domain Dialogue Evaluation Metric using Density Estimation

Despite the recent advances in open-domain dialogue systems, building a reliable evaluation metric is still a challenging problem. Recent studies proposed learnable metrics based on classification models trained to distinguish the correct response. However, neural classifiers are known to make overly confident predictions for examples from unseen distributions. We propose DEnsity, which evaluates a response by utilizing density estimation on the feature space derived from a neural classifier. Our metric measures how likely a response would appear in the distribution of human conversations. Moreover, to improve the performance of DEnsity, we utilize contrastive learning to further compress the feature space. Experiments on multiple response evaluation datasets show that DEnsity correlates better with human evaluations than the existing metrics. Our code is available at https://github.com/ddehun/DEnsity.

==> resources/casestudy_table_deprecated.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}

\setlength\heavyrulewidth{0.25ex}
\newcolumntype{Y}{>{\centering\arraybackslash}X}

\begin{table}[]
\centering
\resizebox{\columnwidth}{!}{%
\begin{tabularx}{\columnwidth}{ c *{3}{Y}}
\toprule
BLEU & USL-H & USR-R \\
Holistic & Human & Ours \\ \hline \\[-2.0ex] \hline
\multicolumn{3}{l}{\begin{tabular}[c]{@{}l@{}}\textbf{A}: Do you want any meat today, Mrs. bird?\\ \textbf{B}: Do you want beef or lamb?\\ \textbf{(Reference)} Beef, please.\\ \textbf{(Model)} Sticks, please.\end{tabular}} \\ \hdashline
1.00(1.00) & 0.60(0.49) & 0.96(0.61) \\
0.70(0.37) & 0.25(0.26) & \textbf{0.39(0.32)} \\ \hline & \\[-2.0ex] \hline
\multicolumn{3}{l}{\begin{tabular}[c]{@{}l@{}}\textbf{A}: I think it's running late.\\ \textbf{B}: It should've been here 30 minutes ago.\\ \textbf{A}: It should be coming soon.\\ \textbf{B}: It better, because I'm already late for work.\\ \textbf{A}: I can't stand riding the bus.\\ \textbf{(Reference)} Me too, it's too unreliable.\\ \textbf{(Model)} Shall I take a bus to get there?\end{tabular}} \\ \hdashline
0.00(0.00) & 0.47(0.34) & 0.97(0.63) \\
0.86(0.83) & 0.08(0.14) & \textbf{0.11(0.12)} \\ \hline & \\[-2.0ex] \hline
\multicolumn{3}{l}{\begin{tabular}[c]{@{}l@{}}\textbf{A}: I need to go to the bank.\\ \textbf{(Reference)} But they are closed today.\\ \textbf{(Model)} Okay. I'll take you there. \end{tabular}} \\ \hdashline
0.00(0.59) & 0.63(0.59) & 0.27(0.20) \\
0.68(0.35) & 1.00(0.86) & \textbf{0.95(0.73)} \\ \hline & \\[-2.0ex] \hline
\multicolumn{3}{l}{\begin{tabular}[c]{@{}l@{}}\textbf{A}:  I did learn that.\\ \textbf{B}: So, then why did you speed up?\\ \textbf{A}: I don't know what to tell you.\\ \textbf{B}: I'm going to have to write you a ticket.\\ \textbf{A}: I understand.\\ \textbf{(Reference)} Here you go. Don’t do that again.\\ \textbf{(Model)} And you'll have to pay a fine.\end{tabular}} \\ \hdashline
0.00(0.72) & 0.65(0.72) & 0.65(0.32) \\
0.80(0.66) & 1.00(0.86) & \textbf{0.98(0.82)} \\ \bottomrule
\end{tabularx}%
}
\caption{Captionss..}
\label{tab:case-study}
\end{table}





==> resources/fig2.tex <==
% % Please add the following required packages to your document preamble:
% \newcommand*{\talign}[2]{% 
%   #1 & : #2 \\
% }

\setlength\heavyrulewidth{0.25ex}
\begin{table}[t!]
\small
\centering
\resizebox{\columnwidth}{!}{%
\begin{tabular}{l}
\toprule
\textbf{A}: We're thinking about going to Toronto.\\ 
\textbf{B}: Have you thought about the cost?\\
\noalign{\vskip 0.3ex} 
\hdashline 
\noalign{\vskip 0.6ex}
\textbf{Answer}: Not yet.\\ 
\textbf{Random}: \underline{This is Mr. Peng speaking.}\\ 
\textbf{Repetition}: Not \underline{yet yet yet yet} yet.\\ 
\textbf{Speaker-Sensitiveness}: \underline{Have you thought} \\ \underline{about the cost?} Not yet.\\ 
\textbf{Contradiction}: \underline{We’re thinking about going}\\
\underline{to Dublin.}\\
\noalign{\vskip 0.3ex} 

\bottomrule
\end{tabular}%
}
\caption{Examples of different adversarial responses along with the original answer response. \textbf{Speaker} denotes a \textit{Speaker-sensitiveness} attack type. Words added to the answer response are marked with \underline{underline}.} 
\label{tab:attack_example}
\vspace{-0.3cm}
\end{table}

